Guiding the Search Towards Failure-Inducing Test Inputs Using Support Vector Machines

In this paper, we present NSGA-II-SVM (Non-dominated Sorting Genetic Algorithm with Support Vector Machine Guidance), a novel learnable evolutionary and search-based testing algorithm that leverages Support Vector Machine (SVM) classification models to direct the search towards failure-revealing test inputs. Supported by genetic search, NSGA-II-SVM creates iteratively SVM-based models of the test input space, learning which regions in the search space are promising to be explored. A subsequent sampling and repetition of evolutionary search iterations allow to refine and make the model more accurate in the prediction. Our preliminary evaluation of NSGA-II-SVM by testing an Automated Valet Parking system shows that NSGA-II-SVM is more effective in identifying more critical test cases than a state of the art learnable evolutionary testing technique as well as naive random search.

==> conferences.tex <==
ISSTA 2023

https://conf.researchr.org/home/issta-2023

May 11, 2023 7:59am EDT (1:59pm your time) - Submissions must be ready by this deadline to be reviewed. 

Mon 17 - Fri 21 July 2023
------------------

ITSC 2023

26th IEEE International Conference on Intelligent Transportation Systems

https://2023.ieee-itsc.org/

May 15, 2023 – Submission deadline for regular, special session, and workshop papers

Bilbao, Spain | September 24-28, 2023

==> content/lessons.tex <==
\section{Discussion}
\label{sec:lessons}

In this section, we briefly discuss the limitations and possible improvements of the proposed testing technique.

In our evaluation, we employ rejection sampling to explore test inputs in the predicted region by the SVM model, i.e., we sample in the whole search space until the required number of samples is found within SVM boundaries. Even though we do not need to evaluate in the simulator every sample, sampling in a high dimensional search space with relatively small failure-revealing regions can be time-consuming \cite{luke2012essentials}. 

The execution time of \algo further depends on the time for the parameter tuning using grid search. As shown by Lameski et al. \cite{Lameski2015gridsearch}, heuristic search approaches are viable alternatives for finding parameters for more accurate SVM models.

% Considering our evaluation, we did not report the number of failing test cases found by our search algorithm, as comparing two test approaches based on these numbers can be misleading. Two test inputs being close can point to a similar testing scenario as discussed already by Nejati et al. \cite{nejati2023reflections}. While a distinctness relation can be defined, choosing appropriate thresholds is complicated.

% To evaluate the performance \algo, we relied only upon search-based engineering QIs. It is further possible, to assess the guidance of the model by reporting the ratio between the number of failing test inputs and all sampled tests in predicted SVM regions. An increasing ratio with an increasing number of SVM iterations should indicate an improving accuracy of the learned failure-inducing region and thus improved guidance by the SVM.



% \begin{itemize}
% \item Selection of Kernel Function
% \item Costly Sampling inside SVM region (but no additional simulation required!)
% \item Evaluation with other CS required
% \item Learning bias; Other classification techniques such as kNN
% \item Cross Validation
% \end{itemize}

==> misc/input_niklas.tex <==

\section{SVM Guided Testing}
\label{sec:approach}

In this paper we propose the \textit{\algolong} (\algo) a search-based testing algorithm that combines evolutionary search with SVM model learning to guide the search towards failure-revealing test cases. \autoref{algo:svm-full} describes the main steps of \algo.

Our proposed algorithm receives a specification of an SBST-Problem as input, containing the system under test (SUT) $S$, the search domain $D$, the fitness function $F$, which is optimized by the NSGA-II algorithm and the oracle function $O$, that labels all evaluated scenarios as failure-revealing or non failure-revealing. NSGA-II-SVM receives three numerical values $n$, $g$ and $i_{max}$ indicating the size of the NSGA-II population, the number of samples, which are generated every iteration using the SVM model and the total number of iterations for the algorithm.

A random initial population $P$ is generated using Latin Hypercube Sampling (LHS), which ensures a uniform distributed starting population. After evaluating the starting population, every iteration of \algo the $n$ best failure-revealing scenarios $Q$, are selected from $P$. All critical scenarios in $P$ are ranked according to their fitness value and the best $n$ are chosen. Then \nsga searches the search domain $D$ for $g$ iterations, generating new samples from $Q$. After evaluating all scenarios the resulting population $Q'$ is joined with $P$. We then classify all scenarios in $P$ as critical or non-critical, separating them in $C^+, C^-$. The SVM algorithm then uses these sets to train its model. The values $(x_1, \ldots, x_n) \in D$ for all points in $C^+, C^-$ are used as features and the criticality label is the target. Since the distribution of all critical samples in $D$ can be highly non-linear, we choose a kernel function to achieve higher accuracy. Our chosen $RBF$ kernel has two hyper-parameters $C_{RBF}$ and $\gamma$ \Lev{@Niklas. Pls explain the parameters.}, which are optimized using grid-search, over a logarithmic scale of variable values. Then, the trained model $M$ is used to sample $s$ new points in the predicted critical regions. We evaluate all new scenarios $R$ and merge them with the total population $P$. This concludes one iteration of NSGA-II-SVM. The algorithm stops after $i_{max}$ iterations and returns all found failure-revealing scenarios $C^+$, from the last iteration.

% \begin{itemize}
%     \item Describe all steps.
%     \item Mention grid search for C and Gamma for SVM Model tuning RBF
% \end{itemize}

\begin{algorithm}[t]
%\small
%\SetAlgoLined
\DontPrintSemicolon
\footnotesize
%\SetNoFillComment

    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{
        $(S, D, F, O)$: An SBST Problem \newline
        $n$: Population size \nsga \newline
        $g$: Generation number \nsga  \newline
        $s$: Random samples to generate in SVM-region
        % $i_{max}$: Number of SVM iterations
    }
    \Output{ $C^+$: critical test cases.}
    \BlankLine
    % $A = \lbrace \rbrace$\tcc*{All evaluated test cases}
    $P \gets initialPopulation(D, n)$\tcc*{Generate initial population}
    $evaluate(P, F, S)$\tcc*{Evaluate initial population by simulation}
    %\BlankLine
    \While{$search\_budget\_available$}{
        $Q \gets non\_dom\_critical(P, n)$\tcc*{Select best, critical n solutions} 
        $Q'\gets \textsc{\nsga}(Q, D, F, S, n,g )$
        \tcc*{Perform genetic search} 
        % \tcc*[l]{Inputs passed to $NSGA-II$:\newline
        %     $(\mathcal{W}, \mathcal{A}, \mathcal{C})$: the ADAS specification;\newline
        %     $p$: current population;\newline
        %     $i_{gen}$: number of samples to be generated; and\newline
        %     $\mathcal{F}_{fit}$: search fitness function.\newline
        %     Outputs received from $NSGA-II$:\newline
        %     $p^\prime$: new samples generated during search.
        %     }
        $P\gets P \cup Q'$\;
        $C^+, C^- \gets do\_label(P,O)$\tcc*{Assign labels whether failing or not.}
        $M \gets SVM(C^+,C^-)$\tcc*{Train SVM model to predict failing regions}
        % \tcc*[l]{Input passed to $SVM$:\newline
        %     $C^+, C^-$: all so far evaluated failing and not failing test cases\newline
        %     Outputs received from $SVM$:\newline
        %     $M$: Model of the search space with decision boundary. \bewline
        %     }
        $R \gets sample(M, s)$ \tcc*[r]{Sample in predicted critical.}
        $evaluate(R,S,F)$\tcc*{Evaluate new samples R by simulation} 
        $ P  \gets P \cup R$ \;
        % $i\ += 1$
    }
    \KwRet{$C^+$}
\caption{NSGA-II-SVM}\label{algo:svm-full}
\end{algorithm}

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.25]{figures/algorithm/svm_boundary_1.png}
%     \caption{Visualization of Step 1}
%     \label{fig:enter-label}
% \end{figure}



% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.2]{figures/todo.png}
%     \caption{Visualization of Step 2}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure*}[!t]
     \begin{subfigure}[b]{0.25\textwidth}
        \label{fig:cigd_example_1}
        \centering
        \includegraphics[width=0.87\textwidth]{figures/algorithm/kernel_svm_1a.pdf}

        % \includegraphics[width=1\textwidth]{results/AVP/trials/NSGAII_Filter/3_runs/NLSGAII/run_2/_Adapted Distance_Velocity (negated).pdf}
        \caption{}
    \end{subfigure}
     \hspace{-1em}
    \begin{subfigure}[b]{0.25\textwidth}
        \label{fig:cigd_example_2}
        \centering
        \includegraphics[width=0.85\textwidth]{figures/algorithm/kernel_svm_2a.pdf}
        % \includegraphics[width=\textwidth]{results/AVP/trials/NSGAII_Filter/3_runs/NSGAII_Filtered/run_3/_Adapted Distance_Velocity (negated).pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.25\textwidth}
        \label{fig:cigd_example_2}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/algorithm/kernel_svm_3a.pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.25\textwidth}
        \label{fig:cigd_example_2}
        \centering
        \includegraphics[width=0.85\textwidth]{figures/algorithm/kernel_svm_4.pdf}
        \caption{}
    \end{subfigure}
    \caption{Overview of the main steps of \algo. a) Explorative search using genetic operations on test inputs with \nsga. b) Generation of an SVM-model based on all so far evaluated test cases and sampling inside the region predicted by the SVM model. c) Repeated exploration by performing genetic operations on best solutions with \nsga. d) Learning a refined SVM-model.  Failure-revealing test cases are represented by circles, non-failing test cases are shown as triangles. Squares are not evaluated test cases. 
    }
    \label{fig:os-plots}
\end{figure*}

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.2]{figures/todo.png}
%     \caption{Visualization of Step 3}
%     \label{fig:enter-label}
% \end{figure}

\begin{algorithm}[t]
%\small
%\SetAlgoLined
\DontPrintSemicolon
\footnotesize
%\SetNoFillComment
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{%\Indp
        $(\mathcal{W}, \mathcal{A}, \mathcal{C})$: ADAS specification\newline
        $\mathcal{F}_{fit}$: Search fitness function\newline
        $\mathcal{C}_{crit}$: Criticality function\tcc*[f]{Labels scenarios as critical/non-critical}\newline
        $i_{gen}, i_{svm}$: Number of new samples generated by NSGA-II and SVM respectively, per iteration\newline
        $n_{inital}, n_{max}$: Size of initial population and total maximum population
    }
    \Output{$p$: Final population.}
    \BlankLine
    $p \gets LHS(n_{initial})$\tcc*{Initial population}
    $evaluate(p, \mathcal{C}_{crit})$\tcc*{Evaluate initial population}
    \BlankLine
    \For{$|p|\leq n_{max}$}{
        $p^\prime \gets NSGA-II((\mathcal{W}, \mathcal{A}, \mathcal{C}), p, i_{gen}, \mathcal{F}_{fit})$\;
        \tcc*[l]{Inputs passed to $NSGA-II$:\newline
            $(\mathcal{W}, \mathcal{A}, \mathcal{C})$: the ADAS specification;\newline
            $p$: current population;\newline
            $i_{gen}$: number of samples to be generated; and\newline
            $\mathcal{F}_{fit}$: search fitness function.\newline
            Outputs received from $NSGA-II$:\newline
            $p^\prime$: new samples generated during search.
            }
        $evaluate(p^\prime, \mathcal{C}_{crit})$\tcc*{Evaluate new samples from $NSGA-II$}
        $p \gets p \cup p^\prime$\;
        $p^{\prime\prime} \gets SVM_{RS}(p, i_{svm})$\;
        \tcc*[l]{Inputs passed to $SVM_{RS}$:\newline
            $p$: current population; and\newline
            $i_{svm}$: number of samples to be generated.\newline
            Outputs received from $SVM_{RS}$:\newline
            $p^{\prime\prime}$: new samples generated during search.
            }
        $evaluate(p^{\prime\prime}, \mathcal{C}_{crit})$\tcc*{Evaluate new samples from $SVM_{RS}$}
        $p \gets p \cup p^{\prime\prime}$\;
    }
\KwRet{$p$}
\caption{NSGA-II-SVM}\label{algo:svm-full}
\end{algorithm}
